Superstrings in General Backgrounds

The thesis divides into three parts. The first is devoted to a careful study of very convenient superspace conventions which are a basic tool for the second part. A theorem is formulated that gives a clear statement about when the signs of a superspace calculation can be omitted. The second part describes the type II superstring using Berkovits' pure spinor formalism. The derivation of the supergravity constraints from classical BRST invariance of Berkovits and Howe is carefully reviewed and new aspects are added. The present derivation uses a covariant variation principle and stays throughout in the Lagrangian formalism. A new result is the explicit form of the BRST transformation of the worldsheet fields for type II. By further deriving the form of the local supersymmetry transformations of the fermionic fields, a connection is established to the starting point of those supergravity calculations, which derive generalized Calabi Yau conditions from effective four-dimensional supersymmetry. Generalized complex geometry is in turn the motivation for the last part, which is based on the author's paper on derived brackets from sigma models and the relation to integrability of generalized complex structures. Finally there are detailed appendices on geometric brackets, generalized complex geometry, Noether's theorem, Bianchi identities, supergauge transformations and the WZ gauge, gamma-matrices and on some aspects of structure group connections.

==> makebst.tex <==
%%
%% This is file `makebst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% makebst.dtx  (with options: `program,optlist,')
%% =============================================
%% IMPORTANT NOTICE:
%% This is a generated file.
%% 
%% It is subject to the same copyright conditions (see below)
%% as in the original file: makebst.dtx.
%% It may not be distributed without makebst.dtx.
%% 
%% Full documentation can be obtained by LaTeXing that original file.
%% Only a few abbreviated comments remain here to describe the usage.
%% =============================================
%% Copyright 1993-2003 Patrick W Daly
%% Max-Planck-Institut f\"ur Aeronomie
%% Max-Planck-Str. 2
%% D-37191 Katlenburg-Lindau
%% Germany
%% E-mail: daly@linmpi.mpg.de
%%
%% With additions by Arthur Ogawa
%% E-mai: ogawa@teleport.com
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt; either
%% version 1 of the License, or any later version.
%%
%% This is a contributed file to the LaTeX2e system.
%% -------------------------------------------------
\def\ProvidesFile#1 [#2 #3 #4]{\def\filename{#1}%
  \def\fileversion{#3}\def\filedate{#2}}
 \ProvidesFile{makebst}
    [2003/09/08 4.1 (PWD, AO)]
 % This file is to be run under TeX (or even LaTeX)
 % It interactively asks questions about the bibliographic style file
 % that you want to produce. When it is finished, it writes a docstrip
 % driver file that produces that .bst file from the generic .mbs that
 % you specified; optionally, it will call the docstrip run immediately.
 % For details, read the documentation in the source file makebst.dtx.
 %--------------------------------------------------------------------
\newwrite\outfile
\newread\ttyin
\newread\infile
\newwrite\ttyout
\def\mes{\immediate\write\ttyout}
\def\wr#1{\immediate\write\outfile{#1}}
\def\umes#1{\mes{^^J#1}\wr{\pc#1}}%
\newlinechar=`\^^J
\def\MBswitch{\catcode`\{=12 \catcode`\}=12
              \catcode`\(=1 \catcode`\)=2\relax}
\def\defpar{\par}
\def\remblk#1 @@{#1}
\def\ask#1#2{\mes{#2}\read\ttyin to #1\ifx#1\defpar\def#1{}\else
   \edef#1{\expandafter\remblk#1@@}\fi}
\def\groot#1.#2@@{#1}
\def\getroot#1{\expandafter\groot#1.@@}
\def\gext#1.#2.#3@@{#2}
\def\getext#1{\expandafter\gext#1..@@}
\def\MBaskfile#1(#2.#3)#4#5{%
\loop
  \def\ans{#2.#3}
\if!#2!
 \if!#3!\ask{#5}{#1}\fi
  \ask{#5}{#1 (default extension=#3)}\else
  \ask{#5}{#1 (default=\ans)}
\fi
  \ifx#5\empty \edef#5{\ans}\fi
  \edef\froot{\getroot#5}
  \edef\fext{\getext#5}
  \ifx\fext\empty \def\fext{#3}\fi
  \edef#5{\froot.\fext}
\if#4i
  \def\temp{Cannot find file `#5'}
  \openin\infile#5\relax
  \ifeof\infile \def\ans{}\fi \closein\infile
\else
 \def\temp{There is no default}
 \ifx\froot\empty \def\ans{}\fi
\fi
  \ifx\ans\empty \mes{*** \temp}
\repeat}
{\catcode`\%=12
 \gdef\pc{%}
 \gdef\pcpc{%% }
}
\def\spsp{\space\space}
\newcount\hours
\newcount\minutes
\def\SetTime{\hours=\time
        \global\divide\hours by 60
        \minutes=\hours
        \multiply\minutes by 60
        \advance\minutes by-\time
        \global\multiply\minutes by-1 }
\SetTime
\def\now{\number\hours:\ifnum\minutes<10 0\fi\number\minutes}
\def\today{\number\year/\ifnum\month<10 0\fi\number\month
   /\ifnum\day<10 0\fi\number\day}
\def\Now{\today\space at \now}
\def\optdef#1#2#3#4{%
  \expandafter\def\csname opt@#1\endcsname{#2}%
  \expandafter\def\csname txt@#1\endcsname{#3}%
  \expandafter\def\csname cmt@#1\endcsname{#4}%
  \edef\optlist{\optlist#1,}%
  \def\OptAns{#1}%
  \mes{(#1) #3\space #4}%
}
\def\optlist{}
\def\nxtopt#1,#2@@{#1} \def\rstopt#1,#2@@{#2}
\newif\ifsw
\def\getans{%
 \edef\optlist{\optlist\pc,}%
 \ask{\ans}{\spsp Select:}%
  \expandafter\ifx\csname opt@\ans\endcsname\relax
  \def\ans{*}%
 \fi
 \expandafter\ifx\csname opt@\ans\endcsname\relax
  \let\ans\OptAns
 \fi
  \edef\ansx{\csname opt@\ans\endcsname}
  \swtrue \loop
    \edef\temp{\expandafter\nxtopt\optlist@@}%
    \edef\optlist{\expandafter\rstopt\optlist@@}%
  \if\temp\pc\swfalse\else
   \if\temp\ans
    \wropt\ans
   \else
    \ifoptlist\wrxopt\temp\fi
      \fi
      \expandafter\let\csname opt@\temp\endcsname\relax
    \fi
  \ifsw \repeat
 \def\optlist{}%
 \ifoptverbose
  \wr{\pc------\string\ans=\ans (==\ansx)-------}%
 \else
   \ifoptlist
     \wr{\pc--------------------}%
   \fi
 \fi
}
\def\wropt#1{%
 \edef\tempx{\csname opt@#1\endcsname}%
 \if!\tempx!
  \wr{\spsp\spsp\pc: (def)
   \csname txt@#1\endcsname
   \ifoptverbose\space\csname cmt@#1\endcsname\fi
  }%
 \else
  \wr{\spsp\tempx,\pc:
   \csname txt@#1\endcsname
   \ifoptverbose\space\csname cmt@#1\endcsname\fi
  }%
 \fi
 \mes{\spsp You have selected: \csname txt@#1\endcsname}%
}
\def\wrxopt#1{%
 \edef\tempx{\csname opt@#1\endcsname}%
 \if!\tempx!
  \wr{\pc\space\spsp\pc: (def)
   \csname txt@#1\endcsname
   \ifoptverbose\space\csname cmt@#1\endcsname\fi
  }%
 \else
  \wr{\pc\space\tempx,\pc:
   \csname txt@#1\endcsname
   \ifoptverbose\space\csname cmt@#1\endcsname\fi
  }%
 \fi
}
\def\beginoptiongroup#1{\begingroup\activatestar\OGcontinue{#1}}%
\def\OGcontinue#1#2{%
 \endgroup
 \begingroup
  \let\OGswitch\secondoftwo\def\tempa{#2}%
  \ifx\tempa\empty\expandafter\firstoftwo\else\expandafter\secondoftwo\fi
  {%
   \activestar
  }{%
   \tempa
  }%
  \OGswitch{}{%
    \let\wropt\wrxopt
    \let\ask\nilans
    \def\mes##1{}%
  }%
  \def\OGmessage{#1}%
  \umes{\ifoptverbose<<\fi\OGmessage}%
}
\def\endoptiongroup{%
  \ifoptverbose\umes{>>\OGmessage}\fi
  \aftergroup\let\aftergroup\ans\expandafter
 \endgroup
 \ans
}
\def\activestar{\let\OGswitch\firstoftwo}
\def\activatestar{\catcode`\*13\relax}
{\activatestar\gdef*{\activestar}}
\def\firstoftwo#1#2{#1}
\def\secondoftwo#1#2{#2}
{\catcode`\$=12\gdef\nilans#1#2{\def\ans{$}}}
\mes{***********************************^^J%
     * This is Make Bibliography Style *^^J%
     ***********************************^^J%
     It makes up a docstrip batch job to produce^^J%
     a customized .bst file for running with BibTeX}

\ask{\yn}{Do you want a description of the usage? (NO)}

\if!\yn!\else\if\yn n\else\if\yn N\else
\mes{In the interactive dialogue that follows,^^J%
     you will be presented with a series of menus.^^J%
     In each case, one answer is the default, marked as (*),^^J%
     and a mere carriage-return is sufficient to select it.^^J%
     (If there is no * choice, then the default is the last choice.)^^J%
     For the other choices, a letter is indicated^^J%
     in brackets for selecting that option. If you select^^J%
     a letter not in the list, default is taken.^^J^^J%
     The final output is a file containing a batch job^^J%
     which may be (La)TeXed to produce the desired BibTeX^^J%
     bibliography style file. The batch job may be edited^^J%
     to make minor changes, rather than running this program^^J%
     once again.}
\fi\fi\fi
\MBaskfile{^^JEnter the name of the MASTER file}(merlin.mbs)i\mfile
\let\mroot=\froot
\let\mext=\fext
\edef\temp{\mroot.opt}
\openin\infile\temp\relax
\let\mnext=\mext
\ifeof\infile\else
  \ask{\yn}{** Warning: a file `\temp' also exists^^J
       \spsp Shall I read it for the menu information? (NO)^^J
       \spsp (Answer `yes' only if you really know what you are doing)}
\if\yn y\def\mnext{opt}\else\if\yn Y\def\mnext{opt}\fi\fi
\mes{Menu information read from `\mroot.\mnext'}
\fi
\closein\infile
\MBaskfile{^^JName of the final OUTPUT .bst file?}(.bst)o\ofile
\let\oroot=\froot
\let\oext=\fext
\ask{\ans}{^^JGive a comment line to include in the style file.^^J%
           Something like for which journals it is applicable.}
\immediate\openout\outfile\oroot.dbj
\wr{\pcpc Driver file to produce \oroot.\oext\space from \mroot.\mext}
\wr{\pcpc Generated with \filename, version \fileversion\space (\filedate)}
\wr{\pcpc Produced on \Now}
\wr{\pcpc}
\wr{\string\input\space docstrip}
\wr{}
\wr{\string\preamble}
\wr{----------------------------------------}
\wr{*** \ans\space ***}
\wr{}
\wr{\string\endpreamble}
\wr{}
\wr{\string\postamble}
\wr{End of customized bst file}
\wr{\string\endpostamble}
\wr{}
\wr{\string\keepsilent}
\wr{}
\wr{\string\askforoverwritefalse}
\begingroup\MBswitch
\wr(\string\def\string\MBopts{\string\from{\mroot.\mext}{\pc)
\endgroup
\newif\ifoptlist
\optlisttrue
\ifoptlist\else
 \ask\yn{Do you want the unused option lines^^J%
         \spsp to appear as comments in the output? (NO)}
 \if!\yn!\else\if\yn n\else\if\yn N\else\optlisttrue\fi\fi\fi
\fi
\newif\ifoptverbose
\ifoptlist
 \ifoptverbose\else
  \ask\yn{Do you want verbose comments? (NO)}
  \if!\yn!\else\if\yn n\else\if\yn N\else\optverbosetrue\fi\fi\fi
 \fi
\fi
\edef\temp{\mroot.\mnext}
\let\endoptions=\endinput
\input\temp
\begingroup\MBswitch
\wr(\spsp}})
\endgroup
\wr{\string\generate{\string\file{\oroot.\oext}{\string\MBopts}}}
\wr{\string\endbatchfile}

\immediate\closeout\outfile
\mes{^^JFinished!!^^J%
     Batch job written to file `\oroot.dbj'}
\def\ofile{\oroot.dbj}
\ask{\yn}{Shall I now run this batch job? (NO)}
\def\temp{\relax}
\if!\yn!\else\if\yn n\else\if\yn N\else
\def\temp{\input\ofile}\fi\fi\fi
{\catcode`\@=11 \ifx\@@end\undefined\else
  \global\let\end=\@@end\fi}
\temp
\end
%% <<<<< End of generated file <<<<<<
%%
%% End of file `makebst.tex'.

